Subgroup growth of right-angled Artin and Coxeter groups

We determine the factorial growth rate of the number of finite index subgroups of right-angled Artin groups as a function of the index. This turns out to depend solely on the independence number of the defining graph. We also make a conjecture for right-angled Coxeter groups and prove that it holds in a limited setting.

==> geometry.tex <==
\subsection{Cube complexes and Salvetti complexes}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Geometric interpretation of the independence number}

Recall that the \emph{crossing graph} of a cube complex is the graph where vertices are the hyperplanes, and two vertices belong to the same edge if and only if the corresponding hyperplanes cross. The following proposition is essentially proved in \cite{HW08}, and we sketch a proof for completeness. 

\begin{prp} \label{crossing}
The graph $\mathcal{G}$ can be obtained as the crossing graph of the Salvetti complex $X_{\art(\mathcal G)}$ associated to $\art(\mathcal G)$. In particular, $\alpha(\mathcal G)$ equals the maximal number of non-intersecting hyperplanes in $X$
\end{prp}

\begin{proof}
Let $B$ be the standard 2-complex of the standard presentation of $\art(\mathcal G)$. Then $B$ is A-special in the sense of \cite{HW08} (see example 3.3 and remark 3.4). The cube complex $B$ is completable and in fact $X_{\art(\mathcal G)}$ is a cube completion of $B$ (see the explanation in Section 2.3 of \cite{HW08}). 

Let $\mathcal G_B$ be the crossing graph of the square complex $B$. In thi paragraph we prove that $\mathcal G_B$ is isomorphic to $\mathcal{G}$. In $B$, each parallelism class consists of a single edge, hence there is a one-to-one correspondence between the set of walls (hence the set of corresponding hyperplanes) and the set of generators of $\art(\mathcal G)$ (hence the set of vertices of $\mathcal{G}$). Furthermore, two hyperplanes cross if and only if the corresponding walls (which are two edges) form a 2-torus in $B$, which happens if and only if the corresponding vertices of $\mathcal{G}$ are connected by an edge. This provides an isomorphism between $\mathcal G_B$ and $\mathcal{G}$. 

On the other hand, there exists a combinatorial map $\tau_A: B \to X_{A(\mathcal G_B)}$, which is called A-typing (see Definition 3.14 and the discussion below in \cite{HW08}). This map gives a local isometry at the level of 2-skeleta. But since $\mathcal G_B$ is isomorphic to $\mathcal{G}$, this induces a local isometry from $B$ to $X^{(2)}_{\art(\mathcal G)}$. 

As above (see also Example 3.3 (2) in \cite{HW08}), in this case the walls of $X_{\art(\mathcal G)}$ are reduced to oriented edges so they are in 1-1 correspondence with the set of generators of $\art(\mathcal G)$. Hence the vertices of the crossing graph $\Gamma_X$ of $X_{\art(\mathcal G)}$ are naturally in 1-1 correspondence with the set of vertices of $\mathcal{G}$. Two hyperplanes in $X_{\art(\mathcal G)}$ cross if and only if their intersection with $X^{(2)}_{\art(\mathcal G)}$ cross in some 2-cell. But since there exists a local isometry from $B$ to $X^{(2)}_{\art(\mathcal G)}$, there exists an edge between two vertices of the crossing graphs of $B$ if and only if there exists an edge between the corresponding vertices of the crossing graph of $X_{\art(\mathcal G)}$. This says that the crossing graph of $X_{\art(\mathcal G)}$ is isomorphic to the crossing graph of $B$, which we already shown to be
isomorphic to $\mathcal G$.
\end{proof}

